Optimal Timing of Moving Target Defense: A Stackelberg Game Model

As an effective approach to thwarting advanced attacks, moving target defense (MTD) has been applied to various domains. Previous works on MTD, however, mainly focus on deciding the sequence of system configurations to be used and have largely ignored the equally important timing problem. Given that both the migration cost and attack time vary over system configurations, it is crucial to jointly optimize the spatial and temporal decisions in MTD to better protect the system from persistent threats. In this work, we propose a Stackelberg game model for MTD where the defender commits to a joint migration and timing strategy to cope with configuration-dependent migration cost and attack time distribution. The defender's problem is formulated as a semi-Markovian decision process and a nearly optimal MTD strategy is derived by exploiting the unique structure of the game.

==> numerical.tex <==
\section{Numerical Results}\label{sec:numerical}
In this section, we study the performance of our algorithms with numerical results. For both continuous and discrete job models, our algorithms achieve clearly higher utility gains compared with commonly adopted heuristics that ignore the heterogeneous multi-resource requirements.

\vspace{1ex}
\noindent {\bf Setup}: We consider a data center with 100 units of CPU and 100 units of memory resources. 100 jobs are generated. The number of job arrivals in each time slot follows a Poisson distribution with a mean of 10, independent of other time-slots. The availability window size of job $j$, that is, $d_j-a_j$, follows an exponential distribution, independent of other jobs. Each job has 100 units of tasks and a parallelism bound of 20. The utility of job $j$ is modeled as a concave function of the form $f_j(x_j) = v_j x_j^\alpha$ with $\alpha<1$. Here, we consider $\alpha = 1/2$ and the coefficient $v_j$ is generated from a uniform distribution in [1,5]. We have also tried other types of concave functions including the logarithmic function and observed similar results. Each job is either CPU-heavy or memory-heavy with equal chance. Each task of a CPU-heavy job requires $R_1$ units of CPU and 1 unit of memory, and each task of a memory-heavy job requires 1 unit of CPU and $R_2$ units of memory, where $R_1$ and $R_2$ are uniformly distributed in $[1,R]$. Each figure below shows the average results over 10 independent scenarios generated for a given set of parameters.

\begin{figure*}[t]
\centering
\subfigure[Continuous tasks with varying availability window size]{
\label{Fig.continuous}
\includegraphics[width=1.65in]{continuous.eps}}
\subfigure[Discrete tasks with varying availability window size]{
\label{Fig.discrete1}
\includegraphics[width=1.65in]{discrete1.eps}}
\subfigure[Discrete tasks with varying resource demand heterogeneity]{
\label{Fig.discrete2}
\includegraphics[width=1.65in]{discrete2.eps}}
\subfigure[Discrete tasks with single resource and unit demand]{
\label{Fig.discrete3}
\includegraphics[width=1.65in]{discrete3.eps}}
\caption{\small Simulation Results. In (a) and (b), $R=8$. In (c), the mean availability window size is 6.}
\label{Fig.result}
\end{figure*}

\vspace{1ex}
\noindent {\bf Continuous Tasks}:
In the continuous setting, we compare Algorithm~\ref{alg:continuous} with the offline optimal and two heuristics. The first heuristic, called s-greedy, always serves the jobs with highest marginal values (subject to the parallelism constraint) and ignores the resource requirements of jobs. The second heuristic, called equal-opp, schedules all the jobs with equal opportunity (subject to the parallelism constraint). Figure~\ref{Fig.continuous} shows the utility gains of these algorithms under different job availability window sizes. We observe that all the algorithms achieve higher utility gains when the availability window size increases, that is when jobs become less delay constrained, which is expected. Algorithm~\ref{alg:continuous} always performs much better than the two heuristics. Moreover, it is close to the offline optimal for smaller availability windows. The gap becomes bigger for large window size due to the deadline oblivious nature of the algorithm.

\vspace{1ex}
\noindent {\bf Discrete Tasks}:
In the discrete setting, we consider two versions of Algorithm~\ref{alg:discrete} that solve the local problem using the local greedy algorithm  (m-greedy for short), and the primal-dual approach (primal-dual for short), respectively. We compare them with the discrete counterparts of the two heuristics in the continuous setting mentioned above. In Figure~\ref{Fig.discrete1}, we again vary the availability window size and observe similar result as in the continuous case. In Figure~\ref{Fig.discrete2}, we vary the value of $R$ that measures the heterogeneity of resource demands. We observe that our algorithms achieve bigger improvement when $R$ becomes larger, which indicates the benefit of being resource aware. We further observe that the two versions of Algorithm~\ref{alg:discrete} have similar performance, which is consistent with our discussion in Section~\ref{sec:discrete_analysis} for small $m$.

We further compare Algorithm~\ref{alg:discrete2} (deadline-aware for short) with the two heuristics in the single resource unit demand setting. We observe that our algorithm achieves a bigger improvement over the greedy algorithm for a larger availability window due to its deadline awareness.  
